DictLLM: Harnessing Key-Value Data Structures with Large Language Models for Enhanced Medical Diagnostics

Structured data offers a sophisticated mechanism for the organization of information. Existing methodologies for the text-serialization of structured data in the context of large language models fail to adequately address the heterogeneity inherent in key-value structured data. These methods are not ideal and frequently result in larger input sizes and poor adaptability to input changes. In this paper, we introduce DictLLM, an innovative framework designed to improve the modeling of key-value structured data, like medical laboratory reports, for generating medical diagnoses. DictLLM integrates three key components: (1) group positional encoding to maintain permutation invariance, (2) hierarchical attention bias to capture the inherent bias in structured data, and (3) an optimal transport alignment layer that aligns the embedding generated by the dictionary encoder with the LLM, thereby producing a sequence of fixed-length virtual tokens. We carry out experiments using various LLM models on a comprehensive real-world medical laboratory report dataset for automatic diagnosis generation, our findings illustrate that DictLLM significantly outperforms established baseline methods and few-shot GPT-4 implementations in terms of both Rouge-L and Knowledge F1 scores. Furthermore, our evaluation of the framework's scalability and robustness, through a series of experiments, underscores its exceptional capability in accurately modeling the complex key-value data structure of medical dictionary data.

==> sections/intro.tex <==
\section{Introduction}

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.5\textwidth]{figures/DictLLM_0_Intro_v3.pdf}
  \caption{Our DictLLM Framework for medical lab report-assisted diagnosis generation. 
  The framework uses a hierarchical dict encoder to encode the medical lab report, and an optimal transport alignment layer to align the embedding generated by the dict encoder and the text encoder.}
  \label{fig:fig_intro}
\end{figure}

Structured data (i.e. graphs, dictionaries, tables), represents an efficient method for organizing information. In the real world, a vast amount of information is neatly contained within these specially structured data formats. (i.e. knowledge graphs, Excel sheets, etc. ) Recently, in the field of natural language processing, employing large language models for the processing of structured data tasks has emerged as a new trend. \citet{TabLLMFewshot-2023} proposes using LLM for few-shot classification tasks on tabular data, \citet{GraphGPTGraph-2023}  proposes using LLM for node classification tasks on graphs, ChatExcel proposed by \citet{KuBiaoChatExcel-2023} use LLM for intelligent question answering tasks on Excel tables. In clinical practice, doctors usually combine medical lab reports with various pieces of information to formulate a patient's final diagnosis. However, current efforts to automate diagnosis generation from daily progress notes using language models, as described in \citet{LeveragingMedical-2023}, still find it challenging to use medical lab reports as essential supporting information for auxiliary diagnoses.

In this paper, we concentrate on one specific type of structured data called medical lab reports and a specific task called lab report-assisted diagnosis generation. Medical lab reports compile patients' laboratory test results using various dictionary structures, a key component in determining the final diagnosis of diseases. Meanwhile, medical laboratory reports are utilized for intricate reasoning tasks, such as automatic diagnosis generation, setting them apart from typical table-based question answering tasks. Selecting this particular type of structured data emphasizes the role of large language models in demonstrating their reasoning capabilities. In lab report-assisted diagnosis generation, both patient information(i.e. medical history, physical examination, etc.), which is written in natural language, and medical lab reports are required to generate the final diagnosis. Distinct from natural language, medical lab reports exhibit two key types of heterogeneity. 

\noindent
\begin{itemize}
  \item Structural heterogeneity: Medical lab reports are organized in a specific structure, characterized by being structured and exhibiting permutation invariance. Specifically, the items within these reports can be interchanged without affecting the overall meaning of the report. In contrast, natural language is unstructured and sequential, where the position of the text cannot be randomly exchanged without altering the meaning.
  \item Information density heterogeneity: Medical lab reports consist of a large amount of sparse and discrete information, while the information in natural language is more compact and coherent.
\end{itemize}


The most common approach currently is to format structured data like medical lab reports as a sequence of tokens, which are then fed into large language models. However, this approach is not designed to explicitly capture most of the above properties. Given the aforementioned differences between medical lab reports and natural language, we raise our research question:\textbf{How could large language model better encode complex, heterogeneous texts like medical lab reports?}

Large language models are trained on natural, sequential text, exhibiting a different inductive bias compared to structured data. So this approach is a suboptimal solution for LLM to process structured data. Moreover, a text serialization approach will lead to large input token size and may exceed the limitation of max token length of large language models, which will limit the scalability of the model. In addition, the text serialization approach is not robust to input perturbation, which is a common phenomenon in medical lab reports.

As shown in Figure \ref{fig:fig_intro}, we propose a novel framework called DictLLM to address the above limitations. DictLLM is a efficient and effective framework for modeling the heterogeneous structure of medical lab reports. Addressing the above three heterogeneities, DictLLM use a carefully designed hierarchical dict encoder, which is based on the SetTransformer \citet{SetTransformer-2019}. To align with the behavior of doctors in actual medical practice, we propose the dict tokenizer that converts detailed numerical values in the laboratory reports into special medical labels. To maintain the permutation invariance of key-value pairs in laboratory reports we propose a group positional encoding to maintain permutation invariance To capture the differences in the correlation between information within and across laboratory reports, we propose incorporating hierarchical attention bias to model the structural inductive bias of medical laboratory reports. We conduct experiment with multiple LLM models on a large scale real-world medical lab report dataset for automatic diagnosis generation. The results show that our proposed framework outperforms the baseline methods and few-shot GPT-4 in terms of both Rouge-L and Knowledge F1 score. Our contributions are summarized as follows:

\noindent
\begin{itemize}
  \item To address the structural heterogeneity, we propose the hierarchical dict encoder to model the structured and permutation invariance of medical lab reports. This encoder effectively captures the structural inductive bias of medical lab reports and achieves better robustness to input perturbation.
  \item To address the information density heterogeneity, we propose the optimal transport alignment layer to align the embedding generated by the dict encoder with the LLM. This layer effectively compress the input token number.
  \item We conduct experiment with multiple LLM models on a large scale real-world medical lab report dataset for automatic diagnosis generation. The results show that our proposed framework outperforms the baseline methods and few-shot GPT-4 in both Rouge-L and Knowledge F1 score.
\end{itemize}

==> tables/main_results.tex <==
\begin{table*}[h]
    \centering
    \small
    \resizebox{\textwidth}{!}{
        \begin{tabular}{ll|ccccccccc}

            \toprule
            \multicolumn{2}{c}{\multirow{2}{*}{Method}}  & \multicolumn{3}{c}{Rouge-L} & \multicolumn{3}{c}{Knowledge}                                                            \\
            \multicolumn{2}{c}{}                         & P                           & R                             & F1    & P              & R     & F1                      \\
            \midrule
            \multirow{3}{*}{\textsc{Zero-shot}}          & internlm-7b                 & 3.59                          & 4.25  & 3.83           & 4.38  & 3.95  & 4.05            \\
                                                         & baichuan-7b                 & 6.14                          & 8.24  & 6.93           & 7.71  & 7.39  & 7.40            \\
                                                         & GPT-4                       & 5.65                          & 32.87 & 8.64           & 8.82  & 28.85 & 12.70           \\
            \midrule
            \multirow{3}{*}{\textsc{Few-shot}}           & internlm-7b                 & 5.89                          & 5.35  & 5.29           & 5.99  & 5.32  & 5.53            \\
                                                         & baichuan-7b                 & 8.35                          & 12.67 & 9.83           & 10.19 & 9.27  & 9.58            \\
                                                         & GPT-4                       & 5.80                          & 33.45 & 8.99           & 9.54  & 32.11 & 13.84           \\
            \midrule
            \multirow{2}{*}{\textsc{Text-Serialization}} & internlm-7b                 & 51.89                         & 45.19 & 46.69          & 50.90 & 46.03 & 47.43           \\
                                                         & baichuan-7b                 & 67.15                         & 63.18 & 63.13          & 67.32 & 64.42 & 64.51           \\
            \midrule
            \multirow{2}{*}{\textsc{\textbf{DictLLM}}}   & internlm-7b                 & 68.67                         & 63.15 & \textbf{64.24} & 68.68 & 64.09 & \textbf{65.24}  \\
                                                         & baichuan-7b                 & 67.26                         & 63.39 & \textbf{63.28} & 67.50 & 64.65 & \textbf{64.61} \\
            \bottomrule
        \end{tabular}
    }
    \caption{
        \textbf{Main Results.}
        We compare the performance of our DictLLM framework with several baseline methods on the medical lab report-assisted diagnosis generation task. We report the Rouge-L and Knowledge F1 scores. The best results are in bold. The detail of the evaluation metrics can be found in section\ref{subsec:metrics}.
    }
    \label{tab:main_results}
\end{table*}

